Les Houches 2017: Physics at TeV Colliders New Physics Working Group Report

We present the activities of the `New Physics' working group for the `Physics at TeV Colliders' workshop (Les Houches, France, 5--23 June, 2017). Our report includes new physics studies connected with the Higgs boson and its properties, direct search strategies, reinterpretation of the LHC results in the building of viable models and new computational tool developments.

==> LLP_DM/tikzfeynman.keys.code.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% TikZ-Feynman
% Feynman Diagrams with TikZ
% Copyright (C) 2015  Joshua Ellis
%
%
% This work may be distributed and/or modified under the conditions of the LaTeX
% Project Public License, either version 1.3 of this license or (at your option)
% any later version.
%
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Joshua Ellis.
%
% This program is distributed in the hope that it will be useful, but WITHOUT
% ANY WARRANTY; without even the implied warranty of MERCHANTABILITY or FITNESS
% FOR A PARTICULAR PURPOSE.  See the LaTeX Project Public License for more
% details.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Shapes
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Crossed Circle
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfdeclareshape{crossed circle}
{
  \inheritsavedanchors[from=circle]
  \inheritanchorborder[from=circle]
  \inheritanchor[from=circle]{north}
  \inheritanchor[from=circle]{north west}
  \inheritanchor[from=circle]{north east}
  \inheritanchor[from=circle]{center}
  \inheritanchor[from=circle]{west}
  \inheritanchor[from=circle]{east}
  \inheritanchor[from=circle]{mid}
  \inheritanchor[from=circle]{mid west}
  \inheritanchor[from=circle]{mid east}
  \inheritanchor[from=circle]{base}
  \inheritanchor[from=circle]{base west}
  \inheritanchor[from=circle]{base east}
  \inheritanchor[from=circle]{south}
  \inheritanchor[from=circle]{south west}
  \inheritanchor[from=circle]{south east}

  \inheritbackgroundpath[from=circle]

  \foregroundpath{
    % Compute south west
    \centerpoint
    \pgf@xc=\radius
    \advance\pgf@x by-0.707107\pgf@xc
    \advance\pgf@y by-0.707107\pgf@xc
    \pgf@xa=\pgf@x \pgf@ya=\pgf@y  % Store coordinates
    % Compute north east point
    \centerpoint
    \pgf@xc=\radius
    \advance\pgf@x by0.707107\pgf@xc
    \advance\pgf@y by0.707107\pgf@xc
    \pgf@xb=\pgf@x \pgf@yb=\pgf@y  % Store coordinates
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@yb}}
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@ya}}
    \pgfsetarrowsstart{}
    \pgfsetarrowsend{}
 }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Decorations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Complete Sines
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Complete sines replaces the path with a whole number of sine waves.
%% Thanks to http://tex.stackexchange.com/a/134516/26980
\pgfdeclaredecoration{complete sines}{initial}
{
  %% Begin by computing the overall path length and find how many sine waves we
  %% can fit in.  Nothing happens beyond the computation.
  \state{initial}[
    width=+0pt,
    next state=move,
    persistent precomputation={
      \def\tikzfeynman@cs@angle@step{30}
      \def\tikzfeynman@cs@current@angle{0}
      \pgfmathsetlengthmacro{\tikzfeynman@cs@points@per@step}{
        \pgfdecoratedinputsegmentlength
        / int(\pgfdecoratedinputsegmentlength
        / \pgfdecorationsegmentlength)
        / 360
        * \tikzfeynman@cs@angle@step}
    },
  ]{}
  %% Move to the origin to the path
  \state{move}[
    width=+\tikzfeynman@cs@points@per@step,
    next state=draw
  ]{
    \pgfpathmoveto{\pgfpointorigin}
  }
  %% Draw the sine wave itself.  This computes the value every 20 degrees and draws straight edges.
  \state{draw}[
    width=+\tikzfeynman@cs@points@per@step,
    switch if less than=1.25*\tikzfeynman@cs@points@per@step to final, % <- bit of a hack
    persistent postcomputation={
      \pgfmathparse{mod(\tikzfeynman@cs@current@angle+\tikzfeynman@cs@angle@step, 360)}
      \let\tikzfeynman@cs@current@angle=\pgfmathresult%
    },
  ]{
    \pgfmathparse{sin(\tikzfeynman@cs@current@angle) * \pgfmetadecorationsegmentamplitude / 2}
    \tikz@decoratepathfalse
    \pgfpathlineto{\pgfqpoint{0pt}{\pgfmathresult pt}}%
  }

  \state{final}{
    \ifdim\pgfdecoratedremainingdistance>0pt\relax
      \pgfpathlineto{\pgfpointdecoratedpathlast}
    \fi
  }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Keys
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\tikzfeynmanset{
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Hooks
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  execute at begin feynman/.code={},
  execute at end feynman/.code={},
  every feynman/.style={/tikzfeynman/every feynman@@/.append style={#1}},
  every feynman@@/.style={
    /tikzfeynman/.cd,
    /tikzfeynman/medium,
  },
  execute at begin feynman@@/.code={}                     %% Internal version
  execute at end feynman@@/.code={},                      %% Internal version
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Diagrams
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  every diagram/.style={/tikzfeynman/every diagram@@/.append style={#1}},
  every diagram@@/.style={
    /tikzfeynman/.cd,
    .search also={/tikz/graphs, /tikz},
    nodes={
      /tikzfeynman/.cd,
      /tikzfeynman/.search also={/tikz/graphs, /tikz},
      /tikzfeynman/every vertex@@,
      /tikzfeynman/every vertex},
    edges={
      /tikzfeynman/.cd,
      /tikzfeynman/.search also={/tikz/graphs, /tikz},
      /tikzfeynman/every edge@@,
      /tikzfeynman/every edge},
    /tikzfeynman/medium,
  },
  every inline/.style={/tikzfeynman/inline@@/.append style={#1}},
  every inline@@/.style={
    /tikzfeynman/small,
  },
  inline/.style={
    /tikz/baseline={#1},
    /tikzfeynman/every inline@@,
  },
  every small/.style={/tikzfeynman/small@@/.append style={#1}},
  every small@@/.style={
    /tikz/node distance=1cm,
    /graph drawing/node distance=1.25cm,
    /graph drawing/level distance=1cm,
    /graph drawing/sibling distance=1.5cm,
    /tikzfeynman/every dot@@/.append style={/tikz/minimum size=1mm},
    /tikzfeynman/every crossed dot@@/.append style={/tikz/minimum size=2mm},
    /tikzfeynman/every blob@@/.append style={/tikz/minimum size=0.5cm},
    /tikzfeynman/arrow size=1.2pt,
    /tikzfeynman/insertion/size=2.5pt,
  },
  small/.style={/tikzfeynman/every small@@},
  every medium/.style={/tikzfeynman/medium@@/.append style={#1}},
  every medium@@/.style={
    /tikz/node distance=1.5cm,
    /graph drawing/node distance=1.9cm,
    /graph drawing/level distance=1.5cm,
    /graph drawing/sibling distance=2.25cm,
  },
  medium/.style={/tikzfeynman/every medium@@},
  every large/.style={/tikzfeynman/large@@/.append style={#1}},
  every large@@/.style={
    /tikz/node distance=2cm,
    /graph drawing/node distance=2.5cm,
    /graph drawing/level distance=2cm,
    /graph drawing/sibling distance=3cm,
    /tikz/graphs/edges={thick},
    /tikzfeynman/every dot@@/.append style={/tikz/minimum size=2mm},
    /tikzfeynman/every crossed dot@@/.append style={/tikz/minimum size=4mm},
    /tikzfeynman/every blob@@/.append style={/tikz/minimum size=1cm},
    /tikzfeynman/arrow size=1.6pt,
    /tikzfeynman/insertion/size=4pt,
  },
  large/.style={/tikzfeynman/every large@@},
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Vertices
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  every vertex@@/.style={
    /tikz/shape=coordinate,
  },
  every vertex/.style={/tikzfeynman/every vertex@@/.append style={#1}},
  vertex/.style={
    /tikzfeynman/every vertex@@,
  },
  every dot@@/.style={
    /tikz/shape=circle,
    /tikz/graphs/as={},
    /tikz/draw,
    /tikz/fill,
    /tikz/inner sep=0pt,
    /tikz/outer sep=0pt,
    /tikz/minimum size=1.5mm,
  },
  every dot/.style={/tikzfeynman/every dot@@/.append style={#1}},
  dot/.style={
    /tikzfeynman/every dot@@,
  },
  every square dot@@/.style={
    /tikz/shape=rectangle,
  },
  every square dot/.style={/tikzfeynman/every square dot@@/.append style={#1}},
  square dot/.style={
    /tikzfeynman/every dot@@,
    /tikzfeynman/every square dot@@,
  },
  every empty dot@@/.style={
    /tikz/fill=none,
  },
  every empty dot/.style={/tikzfeynman/every empty dot@@/.append style={#1}},
  empty dot/.style={
    /tikzfeynman/every dot@@,
    /tikzfeynman/every empty dot@@,
  },
  every crossed dot@@/.style={
    /tikz/fill=none,
    /tikz/shape=crossed circle,
    /tikz/minimum size=3mm,
  },
  every crossed dot/.style={/tikzfeynman/every crossed dot@@/.append style={#1}},
  crossed dot/.style={
    /tikzfeynman/every dot@@,
    /tikzfeynman/every crossed dot@@,
  },
  every blob@@/.style={
    /tikz/shape=circle,
    /tikz/graphs/as={},
    /tikz/draw,
    /tikz/fill=none,
    /tikz/outer sep=0.5\pgflinewidth,
    /tikz/inner sep=0pt,
    /tikz/minimum size=0.75cm,
    /tikz/pattern=north west lines,
  },
  every blob/.style={/tikzfeynman/every blob@@/.append style={#1}},
  blob/.style={
    /tikzfeynman/every blob@@,
  },
  every particle@@/.style={
    /tikz/shape=rectangle,
    /tikz/draw=none,
    /tikz/fill=none,
    /tikz/inner sep=0.3333em,
    /tikz/outer sep=0.5\pgflinewidth,
  },
  every particle/.style={/tikzfeynman/every particle@@/.append style={#1}},
  particle/.style args={#1}{
    /tikzfeynman/every particle@@,
    /tikz/graphs/as={#1},
  },
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Edge styles
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Arrow Style
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  arrow size/.store in=\tikzfeynman@arrow@size,
  arrow size=1.5pt,
  with arrow/.style={
    /tikz/decoration={
      markings,
      mark=at position #1 with {
        \node[
          transform shape,
          xshift=-0.5mm,
          fill,
          inner sep=\tikzfeynman@arrow@size,
          draw=none,
          isosceles triangle
        ] { };
      },
    },
    /tikz/postaction={
      /tikz/decorate=true,
    },
  },
  with reversed arrow/.style={
    /tikz/decoration={
      markings,
      mark=at position #1 with {
        \node[
          transform shape,
          xshift=-0.5mm,
          rotate=180,
          fill,
          inner sep=\tikzfeynman@arrow@size,
          draw=none,
          isosceles triangle
        ] { };
      },
    },
    /tikz/postaction={
      /tikz/decorate=true,
    },
  },
  %% Base Edge Styles
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  every edge@@/.style={},
  every edge/.style={/tikzfeynman/every edge@@/.append style={#1}},
  %% Specific Styles
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  every plain@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw
    },
  },
  every plain/.style={/tikzfeynman/every plain@@/.append style={#1}},
  plain/.style={
    /tikzfeynman/every plain@@,
  },
  every boson@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/decoration={
        complete sines,
        amplitude=1mm,
        segment length=2mm,
      },
      /tikz/decorate=true,
    },
  },
  every boson/.style={/tikzfeynman/every boson@@/.append style={#1}},
  boson/.style={
    /tikzfeynman/every boson@@,
  },
  every charged boson@@/.style={
    /tikzfeynman/with arrow=0.5,
  },
  every charged boson/.style={/tikzfeynman/every charged boson@@/.append style={#1}},
  charged boson/.style={
    /tikzfeynman/boson,
    /tikzfeynman/every charged boson@@,
  },
  every anti charged boson@@/.style={
    /tikzfeynman/with reversed arrow=0.5,
  },
  every anti charged boson/.style={/tikzfeynman/every anti charged boson@@/.append style={#1}},
  anti charged boson/.style={
    /tikzfeynman/boson,
    /tikzfeynman/every anti charged boson@@,
  },
  every photon@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/decoration={
        complete sines,
        amplitude=1mm,
        segment length=2mm,
      },
      /tikz/decorate=true,
    },
  },
  every photon/.style={/tikzfeynman/every photon@@/.append style={#1}},
  photon/.style={
    /tikzfeynman/every photon@@,
  },
  every scalar@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/dashed,
    },
  },
  every scalar/.style={/tikzfeynman/every scalar@@/.append style={#1}},
  scalar/.style={
    /tikzfeynman/every scalar@@,
  },
  every charged scalar@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikzfeynman/with arrow=0.5,
    },
  },
  every charged scalar/.style={/tikzfeynman/every charged scalar@@/.append style={#1}},
  charged scalar/.style={
    /tikzfeynman/scalar,
    /tikzfeynman/every charged scalar@@,
  },
  every anti charged scalar@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikzfeynman/with reversed arrow=0.5,
    },
  },
  every anti charged scalar/.style={/tikzfeynman/every anti charged scalar@@/.append style={#1}},
  anti charged scalar/.style={
    /tikzfeynman/scalar,
    /tikzfeynman/every anti charged scalar@@,
  },
  every ghost@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/dotted,
      /tikz/thick,
    },
  },
  every ghost/.style={/tikzfeynman/every ghost@@/.append style={#1}},
  ghost/.style={
    /tikzfeynman/every ghost@@,
  },
  every fermion@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikzfeynman/with arrow=0.5,
    },
  },
  every fermion/.style={/tikzfeynman/every fermion@@/.append style={#1}},
  fermion/.style={
    /tikzfeynman/every fermion@@,
  },
  every anti fermion@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikzfeynman/with reversed arrow=0.5,
    },
  },
  every anti fermion/.style={/tikzfeynman/every anti fermion@@/.append style={#1}},
  anti fermion/.style={
    /tikzfeynman/every anti fermion@@,
  },
  every majorana@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikzfeynman/with arrow=0.33,
      /tikzfeynman/with reversed arrow=0.73,
    },
  },
  every majorana/.style={/tikzfeynman/every majorana@@/.append style={#1}},
  majorana/.style={
    /tikzfeynman/every majorana@@,
  },
  every anti majorana@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikzfeynman/with reversed arrow=0.33,
      /tikzfeynman/with arrow=0.73,
    },
  },
  every anti majorana/.style={/tikzfeynman/every anti majorana@@/.append style={#1}},
  anti majorana/.style={
    /tikzfeynman/every anti majorana@@,
  },
  every gluon@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/decoration={
        coil,
        aspect=0.75,
        mirror,
        segment length=1.5mm
      },
      /tikz/decorate=true,
    },
  },
  every gluon/.style={/tikzfeynman/every gluon@@/.append style={#1}},
  gluon/.style={
    /tikzfeynman/every gluon@@,
  },
  %% Insertions
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  insertion/.search also={/tikzfeynman,/tikz},
  %% Parameters
  insertion/size/.store in=\tikzfeynman@insertion@size,
  insertion/size=3pt,
  insertion/style/.store in=\tikzfeynman@insertion@style,
  insertion/style={},
  %% Styles
  insertion@@/.style args={[#1]#2}{
    /tikz/decoration={
      markings,
      mark=at position #2 with {
        \tikzfeynmanset{insertion/.cd,#1}
        \draw [\tikzfeynman@insertion@style] (-\tikzfeynman@insertion@size, -\tikzfeynman@insertion@size) -- (\tikzfeynman@insertion@size, \tikzfeynman@insertion@size);
        \draw [\tikzfeynman@insertion@style] (-\tikzfeynman@insertion@size, \tikzfeynman@insertion@size) -- (\tikzfeynman@insertion@size, -\tikzfeynman@insertion@size);
      },
    },
    /tikz/postaction={
      /tikz/decorate=true,
    },
  },
  insertion@@/.default={[]0.5},
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Momentum arrows
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  momentum/.search also={/tikzfeynman,/tikz},
  %% Parameters
  momentum/label distance/.store in=\tikzfeynman@momentum@label@distance,
  momentum/label distance=0pt,
  momentum/arrow distance/.store in=\tikzfeynman@momentum@arrow@distance,
  momentum/arrow distance=3mm,
  momentum/arrow shorten/.store in=\tikzfeynman@momentum@arrow@shorten,
  momentum/arrow shorten=0.15,
  momentum/label style/.store in=\tikzfeynman@momentum@label@style,
  momentum/label style={},
  momentum/arrow style/.store in=\tikzfeynman@momentum@arrow@style,
  momentum/arrow style={},
  %% Styles
  momentum@@/.style args={[#1]#2}{
    /tikz/preaction={
      /tikz/decoration={
        show path construction,
        moveto code={},
        lineto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@1)$)
                node [pos=0.5, auto,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
        curveto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst)
                .. controls (\tikzinputsegmentsupporta) and (\tikzinputsegmentsupportb)
                .. (\tikzinputsegmentlast)
                { \foreach \i in {1, ..., 50} {
                  coordinate [pos=\tikzfeynman@momentum@arrow@shorten + (1-2 * \tikzfeynman@momentum@arrow@shorten)*\i/50] (tf@m@\i) } };
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@2)$)
                foreach \i [count=\j from 3] in {2, ..., 24} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@\j)$)
                }
                -- ($(tf@m@25)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@26)$)
                node [pos=0.5, auto,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@arrow@style] {#2}
                foreach \i [count=\j from 27] in {26, ..., 49} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@\j)$)
                }
                -- ($(tf@m@50)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@49)$);
        },
        closepath code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@1)$)
                node [pos=0.5, auto,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
      },
      /tikz/decorate=true,
    },
  },
  momentum'@@/.style args={[#1]#2}{
    /tikz/preaction={
      /tikz/decoration={
        show path construction,
        moveto code={},
        lineto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@1)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
        curveto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst)
                .. controls (\tikzinputsegmentsupporta) and (\tikzinputsegmentsupportb)
                .. (\tikzinputsegmentlast)
                { \foreach \i in {1, ..., 50} {
                  coordinate [pos=\tikzfeynman@momentum@arrow@shorten + (1-2 * \tikzfeynman@momentum@arrow@shorten)*\i/50] (tf@m@\i) } };
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@2)$)
                foreach \i [count=\j from 3] in {2, ..., 24} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@\j)$)
                }
                -- ($(tf@m@25)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@26)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@arrow@style] {#2}
                foreach \i [count=\j from 27] in {26, ..., 49} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@\j)$)
                }
                -- ($(tf@m@50)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@49)$);
        },
        closepath code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@1)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
      },
      /tikz/decorate=true,
    },
  },
  reversed momentum@@/.style args={[#1]#2}{
    /tikz/preaction={
      /tikz/decoration={
        show path construction,
        moveto code={},
        lineto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast) -- (\tikzinputsegmentfirst)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@1)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
        curveto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast)
                .. controls (\tikzinputsegmentsupportb) and (\tikzinputsegmentsupporta)
                .. (\tikzinputsegmentfirst)
                { \foreach \i in {1, ..., 50} {
                  coordinate [pos=\tikzfeynman@momentum@arrow@shorten + (1-2 * \tikzfeynman@momentum@arrow@shorten)*\i/50] (tf@m@\i) } };
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@2)$)
                foreach \i [count=\j from 3] in {2, ..., 24} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@\j)$)
                }
                -- ($(tf@m@25)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@26)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@arrow@style] {#2}
                foreach \i [count=\j from 27] in {26, ..., 49} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@\j)$)
                }
                -- ($(tf@m@50)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@49)$);
        },
        closepath code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast) -- (\tikzinputsegmentfirst)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@1)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
      },
      /tikz/decorate=true,
    },
  },
  reversed momentum'@@/.style args={[#1]#2}{
    /tikz/preaction={
      /tikz/decoration={
        show path construction,
        moveto code={},
        lineto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast) -- (\tikzinputsegmentfirst)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@1)$)
                node [pos=0.5,
                      auto,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
        curveto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast)
                .. controls (\tikzinputsegmentsupportb) and (\tikzinputsegmentsupporta)
                .. (\tikzinputsegmentfirst)
                { \foreach \i in {1, ..., 50} {
                  coordinate [pos=\tikzfeynman@momentum@arrow@shorten + (1-2 * \tikzfeynman@momentum@arrow@shorten)*\i/50] (tf@m@\i) } };
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@2)$)
                foreach \i [count=\j from 3] in {2, ..., 24} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@\j)$)
                }
                -- ($(tf@m@25)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@26)$)
                node [pos=0.5,
                      auto,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@arrow@style] {#2}
                foreach \i [count=\j from 27] in {26, ..., 49} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@\j)$)
                }
                -- ($(tf@m@50)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@49)$);
        },
        closepath code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast) -- (\tikzinputsegmentfirst)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@1)$)
                node [pos=0.5, auto,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
      },
      /tikz/decorate=true,
    },
  },
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Modifiers
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  half left/.style={
    /tikz/bend left=90,
    /tikz/looseness=1.5,
  },
  half right/.style={
    /tikz/bend right=90,
    /tikz/looseness=1.5,
  },
  quarter left/.style={
    /tikz/bend left=45,
  },
  quarter right/.style={
    /tikz/bend right=45,
  },
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Graceful Failure of LuaTeX keys
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynman@luatex@required@path{
  \PackageWarning{tikz-feynman}{The key you tried to use '\pgfkeyscurrentpath/\pgfkeyscurrentname' requires LuaTeX.  It will be ignored.}
}
\def\tikzfeynman@luatex@required@key{
  \PackageWarning{tikz-feynman}{The key you tried to use '\pgfkeyscurrentpath' requires LuaTeX.  It will be ignored.}
}

\ifluatex\else
  \pgfkeys{
    /graph drawing/.unknown/.code=\tikzfeynman@luatex@required@path,
    /tikz/graphs/.unknown/.code=\tikzfeynman@luatex@required@path,
    /tikz/horizontal/.code=\tikzfeynman@luatex@required@key,
    /tikz/horizontal'/.code=\tikzfeynman@luatex@required@key,
    /tikz/vertical/.code=\tikzfeynman@luatex@required@key,
    /tikz/vertical'/.code=\tikzfeynman@luatex@required@key,
    /tikz/tree layout/.code=\tikzfeynman@luatex@required@key,
    /tikz/spring layout/.code=\tikzfeynman@luatex@required@key,
    /tikz/layered layout/.code=\tikzfeynman@luatex@required@key,
    /tikz/spring electrical layout/.code=\tikzfeynman@luatex@required@key,
    /tikz/electric charge/.code=\tikzfeynman@luatex@required@key,
  }
  % \tikzfeynmanset{
  %   horizontal/.code={The key 'horizontal' requires LuaTeX.  It will be ignored.},
  % }
\fi

\endinput

==> LLP_DM/tikzlibraryfeynman.code.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% TikZ-Feynman
% Feynman Diagrams with TikZ
% Copyright (C) 2015  Joshua Ellis
%
%
% This work may be distributed and/or modified under the conditions of the LaTeX
% Project Public License, either version 1.3 of this license or (at your option)
% any later version.
%
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Joshua Ellis.
%
% This program is distributed in the hope that it will be useful, but WITHOUT
% ANY WARRANTY; without even the implied warranty of MERCHANTABILITY or FITNESS
% FOR A PARTICULAR PURPOSE.  See the LaTeX Project Public License for more
% details.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Pre-requisites
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usetikzlibrary{
  arrows.meta,
  calc,
  decorations,
  decorations.markings,
  decorations.pathmorphing,
  decorations.pathreplacing,
  graphs,
  patterns,
  positioning,
  shapes.geometric,
}
\ifluatex
  \usetikzlibrary{
    graphdrawing
  }
  \usegdlibrary{
    circular,
    force,
    layered,
    trees
  }
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Function definitions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Miscellaneous functions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynman@empty{}

%% Key Manager
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Setup the tikz-feynman key family
\pgfkeys{
  /tikzfeynman/.is family,
  /tikzfeynman/.search also={/tikz},
}

%% |\tikzfeynmanset| allows keys that belong with tikz-feynman to be easily set.
\def\tikzfeynmanset{\pgfqkeys{/tikzfeynman}}

%% Luatex Waring
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Check if we are using luatex
\newif\iftikzfeynman@warn@luatex%
\tikzfeynmanset{
  warn luatex/.is if=tikzfeynman@warn@luatex,
  warn luatex=true,
}

\AtBeginDocument{
  \ifluatex\else
    \iftikzfeynman@warn@luatex
      \PackageWarning{tikz-feynman}{LuaTeX is required if you wish to have vertices automatically placed.  You can disable this warning by setting /tikzfeynman/warn luatex=false}
    \fi
  \fi
}

%% Version check
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Check which version is expected and which is installed
\def\tikzfeynman@compat@parse#1.#2.#3\pgfeov{
  \edef\tikzfeynman@compat@major{#1}
  \edef\tikzfeynman@compat@minor{#2}
  \edef\tikzfeynman@compat@patch{#3}
  \edef\tikzfeynman@compat{#1.#2.#3}
}
\let\tikzfeynman@compat=\tikzfeynman@empty
\pgfkeyslet{/tikzfeynman/compat/.@cmd}{\tikzfeynman@compat@parse}
\ProcessPgfPackageOptions{/tikzfeynman}

\AtBeginDocument{
  \ifx\tikzfeynman@version\tikzfeynman@compat\else
    \ifx\tikzfeynman@compat\tikzfeynman@empty
      \PackageWarning{tikz-feynman}{Consider loading TikZ-Feynman with \string\usepackage[compat=\tikzfeynman@version]{tikz-feynman} so that you can be warned if TikZ-Feynman changes.}
    \else
      \ifx\tikzfeynman@compat@major\tikzfeynman@version@major
        \ifx\tikzfeynman@compat@minor\tikzfeynman@version@minor
          \ifx\tikzfeynman@compat@patch\tikzfeynman@version@patch\else
            \PackageInfo{tikz-feynman}{The preamble requested version \tikzfeynman@compat, but the system version is \tikzfeynman@version.  This should cause no issue.}
          \fi
        \else
          \PackageWarning{tikz-feynman}{The preamble requested version \tikzfeynman@compat, but the system version is \tikzfeynman@version.  This may change some diagrams.}
        \fi
      \else
        \PackageError{tikz-feynman}{The preamble requested version \tikzfeynman@compat, but the system version is \tikzfeynman@version.  They are most likely incompatible.  Please download the appropriate version from jpellis.me/projects/tikz-feynman.}
      \fi
    \fi
  \fi
}

%% Override Lua code if necessary
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynman@apply@patch#1{
  \directlua{require("tikzfeynman.patch.#1.lua")}
}

%% Version 3.0.0, 3.0.1 and 3.0.1a need to be patched.
\ifluatex
  \def\tikzfeynman@temp{3.0.0}
  \ifx\pgfversion\tikzfeynman@temp
    \tikzfeynman@apply@patch{3.0.0}
  \else
    \def\tikzfeynman@temp{3.0.1}
    \ifx\pgfversion\tikzfeynman@temp
      \tikzfeynman@apply@patch{3.0.1}
    \else
      \def\tikzfeynman@temp{3.0.1a}
      \ifx\pgfversion\tikzfeynman@temp
        \tikzfeynman@apply@patch{3.0.1}
      \fi
    \fi
  \fi
\fi

%% Feynman Environment
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Provide `\begin{feynman} ... \end{feynman}` within TikZ pictures.
\tikzaddtikzonlycommandshortcutlet\feynman\tikzfeynman@environment@feynman
\tikzaddtikzonlycommandshortcutlet\endfeynman\endtikzfeynman@environment@feynman

%% \begin{feynman}...\end{feynman}
\def\tikzfeynman@environment@feynman{%
  \pgfutil@ifnextchar[{\tikzfeynman@environment@feynman@opt}
  {\tikzfeynman@environment@feynman@opt[]}}

\def\tikzfeynman@environment@feynman@opt[#1]{%
  \begingroup
  %% Local overrides
  \let\tikz@@scan@fig=\tikzfeynman@scan@fig
  \let\tikzfeynman@orig@graph=\graph
  %% Local commands
  \let\vertex=\tikzfeynman@commands@vertex
  \let\diagram=\tikzfeynman@commands@diagram
  \let\graph=\tikzfeynman@commands@graph
  %% Opening hooks
  \scope
  \tikz@lib@ignore@sizetrue
  \tikzfeynman@tikz@search@tikzfeynman
  \pgfkeys{/tikzfeynman/every feynman@@,#1}
  \pgfkeysvalueof{/tikzfeynman/execute at begin feynman@@}%
  \pgfkeysvalueof{/tikzfeynman/execute at begin feynman}%
}

\def\endtikzfeynman@environment@feynman{%
  %% Closing hooks
  \pgfkeysvalueof{/tikzfeynman/execute at end feynman}%
  \pgfkeysvalueof{/tikzfeynman/execute at end feynman@@}%
  \endscope
  \endgroup
}

%% \feynmandiagram
\def\feynmandiagram{%
  \pgfutil@ifnextchar[{\feynmandiagram@opt}
  {\feynmandiagram@opt[]}}
\def\feynmandiagram@opt[#1]{%
  \pgfutil@ifnextchar[{\feynmandiagram@opt@opt[#1]}
  {\feynmandiagram@opt@opt[#1][#1]}}
\def\feynmandiagram@opt@opt[#1][#2]{%
  \tikz [/tikzfeynman/.cd,#1]
  \graph [/tikzfeynman/.cd,/tikzfeynman/every diagram@@,/tikz/graphs/spring layout,#2]}

%% Allow empty nodes
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\iftikzfeynmanallowemptynode
\newif\iftikzfeynmanvertex
\def\tikzfeynman@scan@fig{%
  \pgfutil@ifnextchar a{\tikz@fig@scan@at}
  {\pgfutil@ifnextchar({\tikz@fig@scan@name}
    {\pgfutil@ifnextchar[{\tikz@fig@scan@options}%
      {\pgfutil@ifnextchar\bgroup{\tikz@fig@main}%
      {\iftikzfeynmanvertex%
         \tikzset{/tikzfeynman/every vertex@@}%
         \iftikzfeynmanallowemptynode%
         \else%
           \tikzset{/tikzfeynman/particle}%
         \fi%
       \fi%
       \tikz@fig@main{}}}}}}%}}

%% Include /tikzfeynman in the search path
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynman@tikz@search@tikzfeynman{%
  \pgfkeys{/tikz/.unknown/.code=%
    \let\tikz@key\pgfkeyscurrentname%
    %% Is it a tikzfeynman key?
    \pgfkeys{/tikzfeynman/\tikz@key/.try={##1}}%
    \ifpgfkeyssuccess%
    \else%
      %% Is it a pgf key?
      \pgfkeys{/pgf/\tikz@key/.try={##1}}%
      \ifpgfkeyssuccess%
      \else%
        \expandafter\pgfutil@in@\expandafter!\expandafter{\tikz@key}%
        \ifpgfutil@in@%
          %% this is a color!
          \expandafter\tikz@addoption\expandafter{\expandafter\tikz@compat@color@set\expandafter{\tikz@key}}%
          \edef\tikz@textcolor{\tikz@key}%
        \else%
          \pgfutil@doifcolorelse{\tikz@key}
          {%
            \expandafter\tikz@addoption\expandafter{\expandafter\tikz@compat@color@set\expandafter{\tikz@key}}%
            \edef\tikz@textcolor{\tikz@key}%
          }%
          {%
            %% Ok, second chance: This might be an arrow specification:
            \expandafter\pgfutil@in@\expandafter-\expandafter{\tikz@key}%
            \ifpgfutil@in@%
              %% Ah, an arrow spec!
              \expandafter\tikz@processarrows\expandafter{\tikz@key}%
            \else%
              %% Ok, third chance: A shape!
              \expandafter\ifx\csname pgf@sh@s@\tikz@key\endcsname\relax%
                \pgfkeys{/errors/unknown key/.expand
                once=\expandafter{\expandafter/\expandafter t\expandafter
                i\expandafter k\expandafter z\expandafter/\tikz@key}{##1}}%
              \else%
                \edef\tikz@shape{\tikz@key}%
              \fi%
            \fi%
          }%
        \fi%
      \fi%
    \fi%
  }
}


%% Vertex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Adapted from |\coordinate| code
\def\tikzfeynman@commands@vertex{
  \path \pgfextra{\tikzfeynmanallowemptynodetrue}
        \pgfextra{\tikzfeynmanvertextrue}
        node}

%% Diagram
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynman@commands@diagram{\@ifstar
  \tikzfeynman@commands@diagram@star%
  \tikzfeynman@commands@diagram@nostar}

\def\tikzfeynman@commands@diagram@nostar{%
  \pgfutil@ifnextchar[{\tikzfeynman@commands@diagram@nostar@opt}
  {\tikzfeynman@commands@diagram@nostar@opt[]}}
\def\tikzfeynman@commands@diagram@nostar@opt[#1]{%
  \tikzfeynman@orig@graph [/tikzfeynman/every diagram@@,/tikz/graphs/spring layout,#1]}

\def\tikzfeynman@commands@diagram@star{%
  \pgfutil@ifnextchar[{\tikzfeynman@commands@diagram@star@opt}
  {\tikzfeynman@commands@diagram@star@opt[]}}
\def\tikzfeynman@commands@diagram@star@opt[#1]{%
  \tikzfeynman@orig@graph [/tikzfeynman/every diagram@@,#1]}

%% Graph
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynman@commands@graph{%
  \pgfutil@ifnextchar[{\tikzfeynman@commands@graph@opt}
  {\tikzfeynman@commands@graph@opt[]}}
\def\tikzfeynman@commands@graph@opt[#1]{%
  \PackageWarning{tikz-feynman}{It is not recommended to use \string\graph.  Use \string\diagram\space or \string\diagram* instead.}
  \tikzfeynman@orig@graph [/tikzfeynman/every diagram@@,#1]}

%% Optional argument in style key
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynman@key@opt#1[#2]#3\pgfeov{%
  \tikzfeynmanset{#1={[#2]#3}}}

%% Insertion
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynman@insertion{%
  \pgfutil@ifnextchar[{\tikzfeynman@key@opt{insertion@@}}
  {\tikzfeynman@key@opt{insertion@@}[]}}
\pgfkeyslet{/tikzfeynman/insertion/.@cmd}{\tikzfeynman@insertion}

%% Momentum
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynman@momentum@std{%
  \pgfutil@ifnextchar[{\tikzfeynman@key@opt{momentum@@}}
  {\tikzfeynman@key@opt{momentum@@}[]}}
\pgfkeyslet{/tikzfeynman/momentum/.@cmd}{\tikzfeynman@momentum@std}

\def\tikzfeynman@momentum@stdp{%
  \pgfutil@ifnextchar[{\tikzfeynman@key@opt{momentum'@@}}
  {\tikzfeynman@key@opt{momentum'@@}[]}}
\pgfkeyslet{/tikzfeynman/momentum'/.@cmd}{\tikzfeynman@momentum@stdp}

\def\tikzfeynman@momentum@stdr{%
  \pgfutil@ifnextchar[{\tikzfeynman@key@opt{reversed momentum@@}}
  {\tikzfeynman@key@opt{reversed momentum@@}[]}}
\pgfkeyslet{/tikzfeynman/reversed momentum/.@cmd}{\tikzfeynman@momentum@stdr}
\pgfkeyslet{/tikzfeynman/rmomentum/.@cmd}{\tikzfeynman@momentum@stdr}

\def\tikzfeynman@momentum@stdrp{%
  \pgfutil@ifnextchar[{\tikzfeynman@key@opt{reversed momentum'@@}}
  {\tikzfeynman@key@opt{reversed momentum'@@}[]}}
\pgfkeyslet{/tikzfeynman/reversed momentum'/.@cmd}{\tikzfeynman@momentum@stdrp}
\pgfkeyslet{/tikzfeynman/rmomentum'/.@cmd}{\tikzfeynman@momentum@stdrp}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Styles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\input tikzfeynman.keys.code.tex

\endinput

==> flavor-rev/LH2017_MB_DG-old.tex <==
%\documentclass[paper=A4,twoside,11pt,DIV=12,headings=big]{scrartcl}
%\pdfoutput=1

%%%% usepackage's %%%%
%\usepackage[a4paper, top=1.2in, bottom=1.2in, left=1.1in, right=1.1in]{geometry}
%\pagestyle{myheadings}
%\usepackage{amsfonts}
%\usepackage{amsmath,amssymb}
%\usepackage[super]{cite}
%\usepackage{graphicx,hyperref}

%%%% macros %%%%
\newcommand{\mailref}[1]{\href{mailto:#1}{#1}}

\newcommand{\Ell}{\mathscr{L}}
\newcommand{\HNP}{\mathscr{H}_{\rm NP}}
\newcommand{\Op}{\mathcal{O}}
\newcommand{\mc}{\mathcal}
\renewcommand{\th}{{\tilde h}}
\newcommand{\tH}{{\tilde H}}
\newcommand{\tphi}{{\tilde \phi}}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
\newcommand{\Bsmumu}{\overline B_s \rightarrow \mu^+ \mu^-}
\newcommand{\re}{{\rm Re}}
\newcommand{\im}{{\rm Im}}
\newcommand{\ra}{\rightarrow}
\newcommand{\alem}{\alpha_{\rm em}}
\newcommand{\sh}{\hat s}
\renewcommand{\th}{\hat t}
\newcommand{\uh}{\hat u}
\newcommand{\mh}{\hat m}
\newcommand{\Mh}{\hat M}
\newcommand{\mumu}{\mu^+ \mu^-}
%\renewcommand{\cite}[1]{[\refcite{#1}]}

\def\sla#1{\setbox0=\hbox{$#1$}\dimen0=\wd0
      \setbox1=\hbox{/} \dimen1=\wd1 \ifdim\dimen0>\dimen1
      \rlap{\hbox to \dimen0{\hfil/\hfil}} #1                        \else
      \rlap{\hbox to \dimen1{\hfil$#1$\hfil}}
      /   \fi}

%\newcommand{\be}{\begin{equation}}
%\newcommand{\ee}{\end{equation}}
%\newcommand{\bea}{\begin{eqnarray}}
%\newcommand{\eea}{\end{eqnarray}}
\newcommand{\nn}{\nonumber}

\newcommand{\tmpbf}[1]{{\bf \boldmath [#1]}}
\newcommand{\tmpbfdg}[1]{{\bf \boldmath \textcolor{red}{[DG: #1]}}}
\newcommand{\tmpcite}{{\bf \textcolor{red}{[cite?]}}}
\newcommand{\tmpred}[1]{\textcolor{red}{#1}}
\newcommand{\tmpblue}[1]{\textcolor{blue}{#1}}
%%%% macros %%%%

%\begin{document}

\chapter{PhysTeV 2017: Review of flavour anomalies}

{\it M.~Borsato, D.~Guadagnoli}

%\thispagestyle{plain}

%%%% TITLE PAGE

%\begin{flushright}
%\small
%LAPTH-004/17
%\end{flushright}

%\begin{center}
%%%% TITLE
%{\sffamily \bfseries \LARGE \boldmath
%PhysTeV 2017: Review of flavour anomalies}\\[0.8 cm]
%%%% AUTHORS
%{\normalsize \sffamily \bfseries Martino Borsato$^a$, Diego Guadagnoli$^b$} \\[0.5 cm]
%\small
%{\em $^a$ Martino's affiliations}\\
%[0.2cm]
%{\em $^b$ Laboratoire d'Annecy-le-Vieux de Physique Th\'eorique UMR5108\,, \\CNRS et Universit\'e de Savoie Mont-Blanc,\\B.P.~110, Annecy-le-Vieux, F-74941 Annecy Cedex, France}
%
%\end{center}

%\begin{abstract}
%
%\noindent The $R_K$ measurement by LHCb suggests non-standard lepton-universality violation (LUV) to occur in $b \to s \ell^+ \ell^-$ decays, with effects in muons rather than electrons. It is intriguing that a number of other measurements of $b \to s \ell^+ \ell^-$ transitions by LHCb and $B$-factories are consistent in magnitude and sign with the $R_K$ effect, and fit a coherent effective-theory picture. Further indications of non-standard LUV are provided by the long-standing discrepancies in $b \to c \tau \nu$ transitions via the ratios $R(D)$ and $R(D^*)$. We review in detail the experimental situation and its rich outlook, the theoretical efforts -- and their challenges -- towards convincing dynamics beyond the effective-theory level, and discuss the many directions of further investigation that propagate from the current situation.
%
%\end{abstract}

%\noindent {\em Keywords:} B-meson decays; theories beyond the Standard Model; hadron colliders; lepton universality
%
%\medskip
%
%\noindent PACS Nos.: 12.15.Ji, 12.60.-i, 13.20.He

\section{Flavour anomalies: theory overview} \label{sec:flavor-th}

\noindent {\bf Introduction --} A whole range of $b \to s$ data involving a $\mumu$ pair display a consistent pattern, with experimental data below the respective Standard-Model (SM) prediction, for di-lepton invariant masses below the charmonium threshold. (An in-depth discussion of the experimental aspects of the measurements is provided separately, in sec. \ref{sec:flavor-exp}.) This is true for the $B^{0} \to K^{0} \mumu$, the $B^{+} \to K^{+} \mumu$ and the $B^{+} \to K^{*+} \mumu$ decays \cite{Aaij:2014pli}, for the $B^0_s \to \phi \mumu$ decay \cite{Aaij:2015esa} and, very recently, even in hyperon channels for the $\Lambda_b \to \Lambda \mumu$ decay \cite{Aaij:2015xza,Detmold:2016pkz}. With these data alone, however, it is presently impossible to establish beyond-SM effects, as branching-ratio measurements suffer in general from sizable theoretical uncertainties due to hadronic form factors. On the other hand, such problem is basically absent if one considers suitable ratios of branching ratios to different lepton channels. Dedicated measurements exist on such ratios, and actually constitute the most alluring set of anomalies. In the $b \to s$ case these measurements are \cite{Aaij:2014ora,Aaij:2017vbb}
\bea
\label{eq:RK}
&R_K([1, 6] {\textrm{GeV}}^2) ~\equiv~ \frac{\mc B (B^+ \to K^+ \mu^+\mu^-)}{\mc B (B^+ \to K^+ e^+e^-)}|_{q^2 \in [1, 6] {\textrm{GeV}}^2} ~=~
0.745^{+0.090}_{-0.074}\,{\textrm{(stat)}}\pm 0.036\,{\textrm{(syst)}}~,&\nn\\
&R_{K^{*0}}([0.045, 1.1] \, {\textrm{GeV}}^2) ~=~ 0.660 ^{+0.110}_{-0.070} \pm 0.024~,&\\
&R_{K^{*0}}([1.1, 6] \, {\textrm{GeV}}^2) ~=~ 0.685 ^{+0.113}_{-0.069} \pm 0.047~,&\nn
\eea
where we have omitted the definition of $R_{K^{*0}}$, analogous to the $R_K$ one, and where $q^2$ denotes the invariant mass squared of the di-lepton pair. All of the above measurements are predicted to be unity (first and third of them) and respectively close to it (second one) within the SM, with a few-percent accuracy \cite{Bordone:2016gaq} (see also \cite{Bobeth:2007dw,Bouchard:2013mia,Hiller:2003js}). Therefore, the $R_{K}$ and $R_{K^{*0}}$ measurements each imply a discrepancy between 2 and $2.6\sigma$ \cite{Aaij:2014ora,Aaij:2017vbb}, at face value signalling lepton-universality violation (LUV) beyond the SM. 

While the electron-channel measurement would be an obvious culprit for the discrepancies, because of bremsstrahlung and lower statistics, disagreement is rather in the muon channel, see \cite{Aaij:2014pli,Aaij:2012vr} and, very recently, ref. \cite{Aaij:2016flj}. The fact that muons are among the most reliable objects within LHCb  would somewhat disfavour systematic effects as an explanation, although of course it cannot be excluded.

Importantly, the emerging picture can be established from ratios alone, but it is supported by the other measurements, whose theory error is more debated. Some comments deserves in particular the $B \rightarrow K^{*} \mu \mu$ angular analysis \cite{Aaij:2013qta,Aaij:2015oid,Abdesselam:2016llu,Wehle:2016yoi,Atlas,CMS}, exhibiting a discrepancy in one combination of the angular-expansion coefficients, known as $P_{5}'$. The theory error on this observable is a matter of debate because, while it is designed to minimize f.f. dependence \cite{Descotes-Genon:2013vna}, what cancels is the dependence on the infinite-$m_b$ form factors. The crucial issue is how important departures from the infinite-$m_b$ limit are as the di-lepton invariant mass squared $q^2$ approaches the charmonium threshold $4 m_c^2$ -- in particular, departures due to $c \bar c$-loop contributions, that at present are still incalculable. Such contributions are formally power suppressed in a $1/m_b$ expansion, but also come with a factor of $1 / (q^2 - 4 m_c^2)$ \cite{Khodjamirian:2010vf}, that becomes larger and larger as $q^2$ approaches the charmonium threshold. On the different approaches towards assigning a significance to the $P_{5}'$ discrepancy, see in particular \cite{Descotes-Genon:2013wba,Lyon:2014hpa,Jager:2014rwa,Ciuchini:2015qxb}. Nonetheless, this observable again supports, even quantitatively, the picture emerging from ratios alone.

Equally interesting results come from measurements of the ratios $R(D^{(*)}) \equiv \mc B (B \to D^{(*)} \tau \nu) / \mc B (B \to D^{(*)} \ell \nu)$ \cite{Lees:2012xj,Aaij:2015yra,Huschle:2015rga,Belle-semilep}. Here the theory error is less intuitive, as the $\tau$ mass is not negligible with respect to $m_B$, and f.f. dependence does not quite cancel in these ratios. However, they can be constrained thanks to accurate LQCD determinations (in the case of $R_D$) \cite{Na:2015kha,Lattice:2015rga} or to other experimental measurements ($R_{D^*}$) \cite{Fajfer:2012vx,Kamenik:2008tj}. Accordingly, a simultaneous fit to all these $R(D)$ and $R(D^*)$ measurements yields a discrepancy with respect to the SM predictions with a significance of about 4$\sigma$ \cite{Amhis:2016xyh}, comparable to the global significance of $b \to s$ anomalies. Note also that $b \to c$ anomalies come jointly from several experiments: $B$ factories and LHCb.

\bigskip

\noindent {\bf Theory considerations --} The above-mentioned discrepancies are intriguing for at least the following reasons: {\em (a)} they concern two sets of observables ($b \to s$ and $b \to c$) related by the SM $SU(2)_L$ symmetry \cite{Bhattacharya:2014wla}; {\em (b)} both $b \to s$ and $b \to c$ measurements suggest dynamics that distinguishes between the different species of leptons, i.e. beyond-SM Lepton-Universality Violation'' (LUV); {\em (c)} discrepancies appear to obey a pattern, i.e. data are always on a given side with respect to the SM predictions; {\em (d)} this pattern finds a straightforward interpretation within what is called an effective-field-theory (EFT) framework, to be expanded upon next.

Let us consider the following Hamiltonian, which is part of the full $\bar b \to \bar s \ell \ell$ one
\bea
\label{eq:HSMNP}
\hspace{-0.3cm}\mc H_{\rm SM+NP}(\bar b \to \bar s\ell^+\ell^-) = -\frac{4G_F}{\sqrt{2}}V_{tb}^* V_{ts}\frac{\alpha_{em}(m_b)}{4\pi} \times \nn \\
\left[\bar b_L \gamma^\lambda s_L \, \bar \ell \left(C_9^{(\ell)} \gamma_\lambda 
 + C_{10}^{(\ell)} \gamma_\lambda \gamma_5\right)\ell \right]  + {\rm H.c.}\,,
\eea
where the index ${(\ell)}$ on the Wilson coefficients $C_{9,10}$ denotes that the corresponding new-physics shift distinguishes between lepton flavours, whereas the SM contribution doesn't, as well known. The SM contributions are such that $C_9 \simeq - C_{10}$ at the $m_b$ scale, yielding (accidentally) an approximate $(V-A) \times (V-A)$ structure. Advocating likewise $C_{9, \rm NP}^{(\mu)} = - C_{10, \rm NP}^{(\mu)}$ for the new-physics shifts (note, in the $\mu$-channel only) turns out to account at one stroke for all $b \to s$ discrepancies \cite{Hiller:2014yaa,Ghosh:2014awa}. Further global fits by different groups consistently show that the by far most favourite solutions are either a negative new-physics (NP) contribution to $C_9$, with $C_{9, \rm NP}^{(\mu)} \sim - 30\% \, C_{9,\rm SM}$, or NP in the mentioned SU(2)$_L$-invariant direction $C_{9, \rm NP}^{(\mu)} = - C_{10, \rm NP}^{(\mu)} \simeq - 12\% \, |C_{9,\rm SM}|$. Note that such a solution is approximately RGE-stable.

The latter solution is especially interesting from a UV point of view, because it amounts to a $(V-A)_{\rm quark} \times (V-A)_{\rm lepton}$ operator (see eq. (\ref{eq:HSMNP})), that can in turn be promoted to an $SU(2)_L$-invariant, which is what one would expect of interactions arising above the EWSB scale. Let us then focus on this solution: $C_9^{(\ell)} \approx - C_{10}^{(\ell)}$ and $|C_{9,\rm NP}^{(\mu)}| \gg |C_{9,\rm NP}^{(e)}|$. Such a pattern, with effects much larger for muons than for electrons, can be generated from a purely third-generation interaction \cite{Glashow:2014iga} 
\begin{equation}
\label{eq:HNP}
\mc H_{\rm NP} = G \, (\bar b_L' \gamma^\lambda b_L') \, (\bar \tau_L' \gamma_\lambda \tau_L')~,
\end{equation}
with $G = 1 / \Lambda_{\rm NP}^2$ a new Fermi-like coupling, corresponding to a NP scale $\Lambda_{\rm NP}$ in the TeV ballpark. The interaction in eq. (\ref{eq:HNP}) is expected, e.g., in partial-compositeness frameworks \cite{Gripaios:2014tna}. The prime on the fields indicates that they are in the ``gauge'' basis, i.e. that below the EWSB scale they need to be rotated to the mass eigenbasis by usual chiral unitary transformations of the form
\bea
\label{eq:U}
b_L' \equiv (d_L')_3 = (U_L^d)_{3i} (d_L)_i~, ~~~~~~~
\tau_L' \equiv (\ell_L')_3 = (U_L^\ell)_{3i} (\ell_L)_i~,
\eea
whereby the r.h.s. fields represent the mass eigenbasis. In the absence of further assumptions on the structure of the rotation matrices, they will in general induce LUV {\em and} Lepton-Flavor Violation (LFV) effects alike \cite{Glashow:2014iga}. This is also a general expectation in a `top-bottom' approach: consider a new, LUV interaction introduced to explain $R_K$, and defined above the electroweak symmetry breaking (EWSB) scale. Such interaction may be of the kind $\bar \ell Z^\prime \ell$, with $Z^\prime$ a new vector boson, or $\bar \ell \phi q$, with $\phi$ a leptoquark. The question arises, in what basis are quarks and leptons in the above interaction. Generically, it is not the mass eigenbasis -- this basis does not yet even exist, as we are above the EWSB scale. Rotation to the mass eigenbasis generates LFV effects, although the initial interaction was introduced to produce only LUV ones.

With the above ingredients we can straightforwardly explain $b \to s$ data. In particular, neglecting the negligible phase-space difference between the electron and the muon channels, one finds
\be
\label{eq:RKmodel}
R_K \approx \frac{|C_9^{(\mu)}|^2 + |C_{10}^{(\mu)}|^2}{|C_9^{(e)}|^2 + |C_{10}^{(e)}|^2} \simeq \frac{2 |C_{10, \rm SM} + C_{10, \rm NP}^{(\mu)}|^2}{2 |C_{10, \rm SM}|^2}~,
\ee
where the factors of 2 on the r.h.s. are due to the contributions from $|C_9|$ and $|C_{10}|$ being equal by assumption. Note as well that
\be
\label{eq:0.77}
0.77 \pm 0.20 = \frac{\mc B(B_s \to \mu \mu)_{\rm exp}}{\mc B(B_s \to \mu \mu)_{\rm SM}} = \frac{\mc B(B_s \to \mu \mu)_{\rm SM + NP}}{\mc B(B_s \to \mu \mu)_{\rm SM}} = \frac{|C_{10, \rm SM} + C_{10, \rm NP}^{(\mu)}|^2}{|C_{10, \rm SM}|^2}~,
\ee
implying, within the model in ref. \cite{Glashow:2014iga}, the correlations (see also \cite{Hiller:2014yaa})
\be
\frac{\mc B(B_s \to \mu \mu)_{\rm exp}}{\mc B(B_s \to \mu \mu)_{\rm SM}} \simeq R_K \simeq \frac{\mc B(B^+ \to K^+ \mu \mu)_{\rm exp}}{\mc B(B^+ \to K^+ \mu \mu)_{\rm SM}}~.
\ee
This relation states that the measurement-over-SM ratio for $\mc B(B_s \to \mu \mu)$ provides a proxy for $R_K$. This is one more good reason to pursue accuracy in the $\mc B(B_s \to \mu \mu)$ measurement. To the extent that the central value on the l.h.s. of eq. (\ref{eq:0.77}) remains low, this test will be a sensitive one already by the end of Run 2, because the $\mc B(B_s \to \mu \mu)$ total error (dominated by the experimental component) is anticipated to be around 10\% \cite{Guadagnoli:2013mru,Bediaga:2012py}.

Concerning the expected LFV, the crucial question of course is whether it is experimentally accessible. The interaction (\ref{eq:HNP}), plus the measured amount of LUV pointed to by $R_K$, provide a general argument \cite{Guadagnoli:2017jcl,Glashow:2014iga} on the LFV rates to expect. In fact, $R_K$ yields the ratio
\be
\rho_{\rm NP} = -0.159^{+0.060}_{-0.070}
\ee
between the NP and the SM+NP contribution to $C_9^{(\mu)}$. Then, for {\em any} decay of the kind $B \to K \ell_i^\pm \ell_j^\mp$, where $i \ne j$ amounts to LFV, one can write
\be
\label{eq:BKll}
\frac{\mc B (B \to K \ell_i^\pm \ell_j^\mp)}{\mc B (B^+ \to K^+ \mu^+ \mu^-)} ~\simeq~ 
2 \rho_{\rm NP}^2 
\frac{| (U^\ell_L)_{3i} |^2 | (U^\ell_L)_{3j} |^2}{|(U^\ell_L)_{32}|^4}~,~~
\ee
where we used the $U$-matrix transformations (\ref{eq:U}), and normalised to the well-measured $\mc B (B^+ \to K^+ \mu^+ \mu^-) \simeq 4.3 \times 10^{-7}$ \cite{Aaij:2014pli}. One thereby obtains
\bea
\label{eq:BKlilj}
\mc B (B \to K \ell_i^\pm \ell_j^\mp) \simeq 5\% \, \cdot \, \mc B (B^+ \to K^+ \mu^+ \mu^-) \, \cdot \, \frac{| (U^\ell_L)_{3i} |^2 | (U^\ell_L)_{3j} |^2}{|(U^\ell_L)_{32}|^4} \simeq &&\nn \\
[0.1cm]
\simeq 2.2 \times 10^{-8} \, \cdot \, \frac{| (U^\ell_L)_{3i} |^2 | (U^\ell_L)_{3j} |^2}{|(U^\ell_L)_{32}|^4}~.\hspace{2.4cm}&&
\eea
Eq. (\ref{eq:BKlilj}) neglects all terms proportional to lepton masses, which in the case of $\tau$ leptons produce corrections of several tens of percent. Such effects are unimportant in the context of the present argument, whose aim is to produce order-of-magnitude estimates. Eq. (\ref{eq:BKlilj}) tells us that LFV $B \to K$ decays are expected to be of order $10^{-8}$ times an {\em unknown factor} involving $U_L^\ell$ matrix entries. Then, the argument about the expected size of LFV effects boils down to an argument about such factor.

In the $\ell_i \ell_j = e \mu$ case, this ratio reads $|(U_L^\ell)_{31} / (U_L^\ell)_{32}| \lesssim 3.7$ \cite{Glashow:2014iga}, implying that the $B \to K \mu e$ rate may be around $10^{-8}$, or much less if $|(U_L^\ell)_{31} / (U_L^\ell)_{32}| \ll 1$. The latter possibility would suggest $U_L^\ell$ entries that decrease in magnitude with the distance from the diagonal. But then one may expect the ratio $|(U_L^\ell)_{33} / (U_L^\ell)_{32}| > 1$, implying a $B \to K \mu \tau$ rate of O($10^{-8}$) or above! In short, assuming the interaction (\ref{eq:HNP}), one can expect just because of the overall unitarity of the $U^\ell_L$ matrix that at least one LFV $B \to K$ decay rate be in the ballpark of $10^{-8}$ \cite{Glashow:2014iga}, which happens to be within reach at LHCb's Run 2.\footnote{For more quantitative studies, see e.g. \cite{Guadagnoli:2015nra,Boucenna:2015raa,Guadagnoli:2016erb}.} An entirely analogous reasoning applies for the purely leptonic modes $B_s \to \ell_i^\pm \ell_j^\mp$.\footnote{%
We should keep in mind that at Run 2 the LHCb is expected \cite{Bediaga:2012py} to provide a first measurement of $\mc B (B_d \to \mu^+ \mu^-)$, which in the SM is as small as $1 \cdot 10^{-10}$.}

Being defined above the EWSB scale, the operator in eq. (\ref{eq:HNP}) can, and should be promoted to a full $SU(2)_L$ invariant \cite{Alonso:2014csa}, as mentioned above. This operation yields interactions of the kind $(\bar Q_L^{\prime i} \gamma^\lambda Q_L^{\prime i})\,(\bar L_L^{\prime j} \gamma_\lambda L_L^{\prime j})$ and $(\bar Q_L^{\prime i} \gamma^\lambda Q_L^{\prime j})\,(\bar L_L^{\prime j} \gamma_\lambda L_L^{\prime i})$, with $i, j$ SU(2)$_L$ indices and $Q_L^\prime$, $L_L^\prime$ the SM quark and lepton doublets in the gauge basis. The second interaction yields in turn charged currents like $(\bar t^\prime_L \gamma^\lambda b_L^\prime)(\bar \tau^\prime_L \gamma_\lambda \nu_{\tau L}^\prime)$. After rotation to the mass eigenbasis, the last structure contributes to $\Gamma(b \to c \tau \nu_\tau)$ \cite{Bhattacharya:2014wla}, thereby allowing to explain the LHCb and $B$-factories deviations on $R(D^{(*)})$.

While the above scenario is very attractive, it has to withstand non-trivial constraints, in particular from $B \to K \bar \nu \nu$ (see also \cite{Calibbi:2015kma}), from LEP-measured $Z \to \ell \ell$ couplings, and, most importantly, from LUV effects in $\tau \to \ell \nu \nu$ decays \cite{Feruglio:2016gvd}. The latter constraints are especially dangerous, as they are tested to per mil accuracy, and they turn out to ``strongly disfavor an explanation of the $R(D^{(*)})$ anomaly  model-independently'' \cite{Feruglio:2016gvd}. The same argument shows that also LFV decays of leptons are generated, and that they provide probes well competitive with the ones pointed out above, in particular $\mc B(\tau \to 3\mu)$, $\mc B(\tau \to \mu \rho) \sim 5 \times 10^{-8}$ \cite{Feruglio:2016gvd}.

\bigskip

\noindent {\bf Model-building considerations --} Up to now we have restricted ourselves to EFT considerations. Needless to say, we would expect the EFT picture to be the result of some new UV dynamics. Progress in this respect has to face a few challenging obstacles. The first one is the fact that, in the SM, $B \to D^{(*)} \tau \nu$ and $B \to K^{(*)} \ell \ell$ decays arise respectively at tree and loop level, whereas the NP corrections hinted at by data are in either case of O(15-25\%). This issue is relevant if we seek a common explanation of $b \to c \tau \nu$ and $b \to s \ell \ell$ discrepancies.

A second obstacle is inherent in the fact that the needed NP is of the kind $J_{\rm q} \times J_{\rm \ell}$, i.e. the product of a quark and a lepton current. In most UV setups, such operators are typically accompanied by $J_{\rm q} \times J_{\rm q}$ and $J_{\rm \ell} \times J_{\rm \ell}$ structures, that are severely constrained by data, respectively from $B_s$-mixing observables, and from purely leptonic LFV or LUV decays.

Finally, a third obstacle emerges from the observation that most model-building attempts advocate new charged, and possibly colored, states, with masses not larger than O(tens of TeV) and with significant couplings to 3$^{\rm rd}$-generation SM fermions. These conditions make constraints from direct searches, in particular of resonances decaying to $\tau \tau$ pairs, especially relevant, see \cite{Greljo:2015mma,Faroughy:2016osc}.

With the above qualifications, many proposals of plausible UV models for the anomalies have been made, typically involving a new Lorentz scalar or vector, with any\footnote{Compatibly with gauge invariance.} of the following transformation properties under the SM gauge group: a singlet or a triplet under SU(3)$_c$ (the latter case is known as leptoquark); a singlet or a doublet or a triplet under SU(2)$_L$.

It follows a very short review of the models proposed to account simultaneously for the $b \to s$ and the $b \to c$ anomalies. This review is far from exhaustive, in particular it limits itself to work published at the time of this workshop (summer 2017). Our aim is primarily to expose the non-trivial challenges that such simultaneous explanation poses in the face of all the existing constraints. 

\bigskip

\noindent {\bf Explicit Models --} A first natural possibility among those mentioned before is that of a color-singlet, weak-triplet vector field, i.e. a heavier replica of the $W^\pm, Z^0$ bosons \cite{Greljo:2015mma,Boucenna:2016wpr}. Ref. \cite{Greljo:2015mma} discusses in detail the bounds imposed by $\tau \to \ell \nu \nu$, $B_s$-mixing, and direct searches. The minimal model turns out to be ruled out by searches of resonance-produced $\tau$ pairs. Non-minimal versions of the model can avoid this constraint at the price of a larger parameter space. Ref. \cite{Boucenna:2016wpr} aims at a general discussion of gauge extensions with LUV, and concludes that within these models universality violation is most likely a signature of Yukawa couplings between the SM fermions and new vector-like fermions. The other color-neutral possibilities (weak triplet of scalars, and weak doublets or singlets) either amount to extended Higgs sectors, that in general have a tree-level FCNC problem, or else fail to fulfil gauge invariance.

Let us now turn to color-triplet scalars or vectors. Color triplets are usually referred to as leptoquarks (LQ) \cite{Davidson:1993qk}, i.e. states coupled to a quark and a lepton. By definition they thus avoid tree-level contributions to meson mixings and purely leptonic LUV/LFV decays. Besides, vector LQs are ubiquitous in grand-unified theory (GUT) scenarios. Ref. \cite{Bauer:2015knc} proposes an $SU(2)_L$-singlet LQ able to explain both $R_{K^{(*)}}$ and $R(D^{(*)})$ with loop corrections to the former and tree corrections to the latter. While such dynamics is rather appealing, in that it reproduces the same suppression pattern as the SM, the model produces too large corrections to the measured ratio $\mc B (B \to D \mu \nu) / \mc B (B \to D e \nu)$ \cite{Becirevic:2016oho}. Ref. \cite{Fajfer:2015ycq} proposes a weak-triplet Lorentz-vector with completely general flavour couplings $g_{ij}$ to a $\bar Q^i_L L^j_L$ bilinear, $i,j$ denoting flavour indices. This scenario generalises \cite{Calibbi:2015kma}, where the LQ is assumed to couple only to the third-generation fermions in the weak basis. From a fit to data, one obtains $g_{b \mu}^* g_{s \mu} \sim 10^{-3} \cdot (M_U/\mbox{TeV})^2$ and $|g_{b \tau}| \gtrsim 2$ from $b \to s$ and respectively $b \to c$ anomalies, with $M_U$ the mass of the LQ. One may argue that this hierarchy introduces another flavour problem. Besides, $M_U \neq 0$ requires a Higgs mechanism.

Ref. \cite{Barbieri:2015yvd} interprets the patterns of corrections required by the anomalies as the result of a broken flavour symmetry. Specifically, the authors note that $b \to c \tau \nu$ anomalies involve the $3^{\rm rd}$ generation of leptons, whereas $b \to s \ell \ell$ ones concern light generations of leptons only. They then invoke a flavour group $G_F$ and a tree-level LQ exchange such that, in the limit of exact $G_F$, the LQ couples only to the $3^{\rm rd}$ generation of SM fermions, and the needed NP effects arise from the $G_F$ breaking. This implies singly suppressed corrections to $b \to c \tau \nu$ and three times suppressed effects in $b \to s \ell \ell$. Ref. \cite{Barbieri:2015yvd} encompasses the cases of a weak-singlet vector, and of a weak-singlet scalar or vector LQ.

While the mechanism is very plausible, the generated EFT operators do not escape, in general, the argument in ref. \cite{Feruglio:2016gvd}, because the only $G_F$-invariant SM fermions are the left-handed doublets. Still, among the merits of ref. \cite{Barbieri:2015yvd} is also the fact that it exposes the strong UV-cutoff sensitivity of LQ models involving a Lorentz vector. This sensitivity manifests itself in the power-like divergence of 2-, 3-point functions, and box diagrams.\footnote{The latter reintroduce at one loop the constraint from $B$-meson mixings, that for LQs is absent at tree level, as mentioned above.} Such cutoff sensitivity cries out an explicit UV completion, if only for the sake of calculability. An attempt in this direction is ref. \cite{Barbieri:2016las}, although a separate challenge is represented by the detailed verification that this UV completion does withstand all the existing constraints.

Finally, ref. \cite{Becirevic:2016yqi} advocates a weak-doublet scalar LQ coupled to the bilinears $\bar d_R L_L$ and $\bar Q_L \nu_R$ through $Y_L$ and $Y_R$ Yukawa couplings, whereby the right-handed $\nu$ field is required to have negligibly small mass. By virtue of the $(V + A)_{\rm quark} \times (V-A)_{\rm lepton}$ current invoked, this setup is not affected by the constraint in ref. \cite{Feruglio:2016gvd}, but predicts $R_{K^*} > 1$, in tension with the recent measurement \cite{Aaij:2017vbb}.

\bigskip

\noindent {\bf Further tests --} The above discussion highlights that the UV aspects of the dynamics responsible for the anomalies are not quite as established as the EFT picture. Of course, if anomalies are here to stay, the correct UV picture will eventually emerge, guided from data. Further tests that can help consolidating the picture may be classified into three broad categories:
\begin{itemize}
\item Measurements of additional LUV ratios;
\item Extraction of long-distance effects from {\em data};
\item Definition and measurement of new observables sensitive to $C_9$ and $C_{10}$.
\end{itemize}
The first direction is rather evident. Other planned measurements include $R_\phi$, $R_{K_0(1430)}$, $R_{f_0}$, and the inclusive $R_{X_s}$. An interesting test \cite{Hiller:2014ula} is to define the double ratios
\be
X_H \equiv \frac{R_H}{R_K}~,
\ee
with $H = K^*,$ $\phi$, $K_0(1430)$, $f_0$ or $X_s$. Deviations from unity in $X_H$ can only come from right-handed quark currents.

As concerns the second item, it should be recalled that, especially in $b \to s \ell \ell$ modes an important obstacle towards a robust comparison of data with theory is the presence of long-distance (LD) effects due to $c \bar c$ loops. (I reiterate, however, that while this may be an issue for branching ratios, it is not for ratios such as $R_K$.) Encouraging is the fact that, in many cases, this matter seems amenable to be sorted out experimentally, by measuring the $m_{\mumu}$ spectrum, including the $c \bar c$ resonances, and fitting it to suitable parameterizations such as \cite{Lyon:2014hpa,Kruger:1996cv,Guadagnoli:2017quo}. An application of this approach to the $B^+ \to K^+ \mumu$ case was recently  presented in ref. \cite{Aaij:2016cbx}. Interestingly, the measurement yields a result compatible with previous measurements \cite{Aaij:2014pli} and, again, {\em below} the SM prediction \cite{Bailey:2015dka}.

Finally, the third item above suggests to pursue measurements of new observables, independently sensitive to $C_9$ and $C_{10}$. One example is the $B_s \to \mumu \gamma$ decay \cite{Dincer:2001hu,Melikhov:2004mk}, whose spectrum is, for low $q^2$, sensitive to electromagnetic-dipole operators, and, in the whole $q^2$ range, to interactions in eq. (\ref{eq:HSMNP}) as well as to their right-handed counterparts. Besides, its total branching ratio is one order of magnitude above the $B_s \to \mumu$ one, since the chiral suppression in the latter decay is replaced by an $\alpha_{\rm em} / \pi$ factor \cite{Dincer:2001hu}. (For this very reason, the radiative decay is promising even for lepton-flavor-violating searches \cite{Guadagnoli:2016erb,Guadagnoli:2017jcl}.) However, a measurement of the $B_s \to \mumu$ decay by direct detection of the photon poses a major challenge at hadron colliders. Ref. \cite{Dettori:2016zff} points out that, for large $q^2$, $B_s \to \mumu \gamma$ events may actually be searched for in the very same event sample selected for the $\mc B(B_s \to \mumu)$ measurement, by enlarging the $q^2$ signal window beneath the peak region $q^2 \simeq m_{B_s}^2$. This method would provide the very first experimental determination of $\mc B(B_s \to \mumu)$.

\section{Flavour anomalies: experimental aspects} \label{sec:flavor-exp}

Here we collect an overview of the main experimental aspects of -- and challenges behind -- the measurements responsible for the anomalies. [Here goes Martino's contribution.]

%\bibliographystyle{JHEP}
%\bibliography{LH2017_MB_DG}

%\end{document}
